brTPF: Bindings-Restricted Triple Pattern Fragments (Extended Preprint)

The Triple Pattern Fragment (TPF) interface is a recent proposal for reducing server load in Web-based approaches to execute SPARQL queries over public RDF datasets. The price for less overloaded servers is a higher client-side load and a substantial increase in network load (in terms of both the number of HTTP requests and data transfer). In this paper, we propose a slightly extended interface that allows clients to attach intermediate results to triple pattern requests. The response to such a request is expected to contain triples from the underlying dataset that do not only match the given triple pattern (as in the case of TPF), but that are guaranteed to contribute in a join with the given intermediate result. Our hypothesis is that a distributed query execution using this extended interface can reduce the network load (in comparison to a pure TPF-based query execution) without reducing the overall throughput of the client-server system significantly. Our main contribution in this paper is twofold: we empirically verify the hypothesis and provide an extensive experimental comparison of our proposal and TPF.

==> ChartsNetworkLoadExperimentsFeasible.tex <==
\begin{figure}[t!]
\vspace*{-12mm} % Layout Adjustment
\centering
	\subfigure[\footnotesize sum of all \numreq\ for the FEASIBLE~runs]{%
		\includegraphics[width=0.47\textwidth]{charts/feasible-varyMaxMpR-numOfRequests-sum}%
		\label{chart:feasible-varyMaxMpR-numOfRequests-sum}%
	}\hfill
	\subfigure[\footnotesize sum of all \dataRecv\ (FEASIBLE~runs)]{%
		\includegraphics[width=0.47\textwidth]{charts/feasible-varyMaxMpR-triplesReceived-sum}%
		\label{chart:feasible-varyMaxMpR-triplesReceived-sum}
	}

	\subfigure[\footnotesize number of queries for which brTPF has a better~(resp.\ same or worse) \numreq\ than TPF]{%
		\includegraphics[width=0.47\textwidth]{charts/feasible-varyMaxMpR-numOfRequests-drillIn}%
		\label{chart:feasible-varyMaxMpR-numOfRequests-drillIn}%
	}\hfill
	\subfigure[\footnotesize number of queries for which brTPF has~a better~(or same, or worse) \dataRecv\ than TPF]{%
		\includegraphics[width=0.47\textwidth]{charts/feasible-varyMaxMpR-triplesReceived-drillIn}%
		\label{chart:feasible-varyMaxMpR-triplesReceived-drillIn}
	}

	\subfigure[\footnotesize breakdown of the number of queries in terms of the differences between \numreq\ of brTPF~(\maxMpR$=$30) and of TPF]{%
		\includegraphics[width=0.47\textwidth]{charts/feasible-varyMaxMpR-numOfRequests-drillInDeeper}%
		\label{chart:feasible-varyMaxMpR-numOfRequests-drillInDeeper}%
	}\hfill
	\subfigure[\footnotesize breakdown of the number of queries in terms of the differences between \dataRecv\ of brTPF~(maxM/R$=$30) and of TPF]{%
		\includegraphics[width=0.47\textwidth]{charts/feasible-varyMaxMpR-triplesReceived-drillInDeeper}%
		\label{chart:feasible-varyMaxMpR-triplesReceived-drillInDeeper}
	}
	\caption{Measurements of network-related metrics using FEASIBLE.}
	\label{charts:feasible-varyMaxMpR-network}
\end{figure}%
